HapPenIng: Happen, Predict, Infer -- Event Series Completion in a Knowledge Graph

Event series, such as the Wimbledon Championships and the US presidential elections, represent important happenings in key societal areas including sports, culture and politics. However, semantic reference sources, such as Wikidata, DBpedia and EventKG knowledge graphs, provide only an incomplete event series representation. In this paper we target the problem of event series completion in a knowledge graph. We address two tasks: 1) prediction of sub-event relations, and 2) inference of real-world events that happened as a part of event series and are missing in the knowledge graph. To address these problems, our proposed supervised HapPenIng approach leverages structural features of event series. HapPenIng does not require any external knowledge - the characteristics making it unique in the context of event inference. Our experimental evaluation demonstrates that HapPenIng outperforms the baselines by 44 and 52 percentage points in terms of precision for the sub-event prediction and the inference tasks, correspondingly.

==> queries/wikidata_queries.tex <==
Wimbledon sub-events

SELECT DISTINCT ?subEvent ?subEventLabel
WHERE 
{
  ?edition wdt:P31 wd:Q41520.
  ?subEvent wdt:P361+ ?edition .
  SERVICE wikibase:label { bd:serviceParam wikibase:language "[AUTO_LANGUAGE],en". }
}

---

Wimbledon editions

SELECT DISTINCT ?edition ?editionLabel
WHERE 
{
  ?edition wdt:P31 wd:Q41520.
  SERVICE wikibase:label { bd:serviceParam wikibase:language "[AUTO_LANGUAGE],en". }
}
